PriMask: Cascadable and Collusion-Resilient Data Masking for Mobile Cloud Inference

Mobile cloud offloading is indispensable for inference tasks based on large-scale deep models. However, transmitting privacy-rich inference data to the cloud incurs concerns. This paper presents the design of a system called PriMask, in which the mobile device uses a secret small-scale neural network called MaskNet to mask the data before transmission. PriMask significantly weakens the cloud's capability to recover the data or extract certain private attributes. The MaskNet is em cascadable in that the mobile can opt in to or out of its use seamlessly without any modifications to the cloud's inference service. Moreover, the mobiles use different MaskNets, such that the collusion between the cloud and some mobiles does not weaken the protection for other mobiles. We devise a {\em split adversarial learning} method to train a neural network that generates a new MaskNet quickly (within two seconds) at run time. We apply PriMask to three mobile sensing applications with diverse modalities and complexities, i.e., human activity recognition, urban environment crowdsensing, and driver behavior recognition. Results show PriMask's effectiveness in all three applications.

==> fig/comparison/gnuplot <==
set terminal postscript eps enhanced color dashed dl 1 font 'Times-New-Roman,14'
#set terminal postscript eps color dashed dl 1 
set output "reconstruction_har.ps"
set size 0.29,0.35
set xrange [0:1.0]
set yrange [0:1.0]
#set format y "%g%%" 
# set format y "%.0f%%"
set xtics 0,0.3,1.2
set ytics 0,0.2,1


#set lmargin 0
# set ytics ("100\%" 100)

# set ytics ("100\\%" 100, "80\\%" 80,"60\\%" 60,"40\\%" 40,"20\\%" 20,"0\\%" 0,)
set style fill solid 0.5 #fillstyle
#set tics nomirror
set key right bottom samplen 1 width -2

set xlabel "Test accuracy" 
set ylabel "Attack success rate" offset 2,0


set style line 1 lc rgb "#FF0055" lt 2 
set style line 2 lc rgb "#2C397D" lt 3 dashtype 3
#set parametric
plot "tradeoff_points.txt" using 1:2 title "PAN" lc rgb "red" lw 3 dt 2,\

set output
reset

==> hypernetwork.tex <==
{\bf HyperNet} \cite{ha2016hypernetworks} is a neural network that, given an input sampled from a latent distribution, outputs parameters of another neural network. In existing studies, HyperNets are used to generate many neural networks for detecting out-of-distribution inputs \cite{henning2018approximating} and adversarial examples \cite{ratzlaff2019hypergan}, and assess the uncertainty on an inference sample \cite{wang2018adversarial,su2020blindly}.
{\blue In \cite{henning2018approximating,tang2021learning}, they use adversarially trained HyperNets to approximate predictive distributions or learn complex policy distribution, correspondingly. However, their discriminators are unified against heterogeneous generated neural network. While in PriMask, we adopt one-to-one matched AttackNets against temporary MaskNets in the training phase, which performs more rational as the simulation of the adversary. }

\begin{comment}
for robust inference. HyperNet-generated ensembles are used to detect inputs that are out of the training data's distribution \cite{henning2018approximating} and maliciously added with adversarial perturbations for misleading the inference \cite{ratzlaff2019hypergan}.
%the goal of training the HyperNet is to generate a large number of diverse target networks for various downstream applications that require an estimate of uncertainty.
%For example, in anomaly detection, the HyperNet-generated ensembles can be used to measure the uncertainty on out-of-distribution data \cite{henning2018approximating}, which is the unseen data that is from a different distribution as that of the training dataset. Similarly, HyperNet can be used for detecting adversarial example \cite{ratzlaff2019hypergan}, which is an extreme type of out-of-distribution data that aims to mislead a victim neural network to yield an erroneous output by adding carefully crafted small perturbations.
In \cite{wang2018adversarial}, the confidence scores of multiple HyperNet-generated inference models are used to assess the uncertainty on the unlabelled samples, which guides the decisions to ask an oracle for labels.
%. For samples with high uncertainties, an external oracle will be queried for labeling the sample. 
%can serve as the acquisition function that gives the model's uncertainty on different unlabelled data points and decides which data points to ask an external oracle for labels, such that the labelling effort required for model training is reduced.
In \cite{su2020blindly}, HyperNet is used for domain adaptation. Specifically, based on the recognized content of an input image, the HyperNet generates a target network to assess the quality of the input image.
%For instance, in the work \cite{su2020blindly}, a HyperNet is used to generate weights for different quality prediction networks according to the recognized content of the input images.
\end{comment}
